OKRidge: Scalable Optimal k-Sparse Ridge Regression

We consider an important problem in scientific discovery, namely identifying sparse governing equations for nonlinear dynamical systems. This involves solving sparse ridge regression problems to provable optimality in order to determine which terms drive the underlying dynamics. We propose a fast algorithm, OKRidge, for sparse ridge regression, using a novel lower bound calculation involving, first, a saddle point formulation, and from there, either solving (i) a linear system or (ii) using an ADMM-based approach, where the proximal operators can be efficiently evaluated by solving another linear system and an isotonic regression problem. We also propose a method to warm-start our solver, which leverages a beam search. Experimentally, our methods attain provable optimality with run times that are orders of magnitude faster than those of the existing MIP formulations solved by the commercial solver Gurobi.

==> sections/Algorithm1_more_detailed.tex <==
\begin{algorithm}
\caption{DetailedBnB($\mathcal{D}$,$k$,$\lambda_2$, $\epsilon$, $T_{\text{iter}}$, $T_{\max}$) $\rightarrow~\bbeta$}
\label{alg:BnB_overview_algorithm}
\begin{flushleft}
\textbf{Input:} dataset $\mathcal{D} = \{ (\bx_i, y_i) \}_{i=1}^n$, sparsity constraint $k$, $\ell_2$ coefficient $\lambda_2$, optimality gap $\epsilon$, iteration limit $T_{\text{iter}}$ (default value is $200$) for subgradient ascent, and time limit $T_{\max}$. \hfill\\
\textbf{Output:} a sparse continuous coefficient vector $\bbeta \in \bbR^p $ with $\lVert \bbeta \rVert_0 \leq k$.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE $\epsilon_{\text{best}}, \calL^{\text{best}}_{\text{lower}}, \bbeta_{\text{upper}}^{\text{best}}, \calL_{\text{upper}}^{\text{best}} = \infty, -\infty, \mathbf{0}, 0$ \COMMENT{Initialize the best optimality gap to be infinity, best lower bound to be negative infinity, best solution to be $\mathbf{0}$, and its corresponding loss to be 0.}
    \STATE $\calQ \leftarrow \text{initialize an empty queue (FIFO) structure}$ \COMMENT{FIFO corresponds to a breadth-first search.}
    \STATE $\calN_{\text{select}} = \emptyset$, $\calN_{\text{avoid}} = \emptyset$ \COMMENT{Coordinates in $\calN_{\text{select}}$ can be selected during heuristic search and lower bound calculation for a node; Coordinates in $\calN_{\text{avoid}}$ must be avoided.}
    \STATE $\text{RootNode} = \text{CreateNode}(\calD, k, \lambda_2, \calN_{\text{select}}, \calN_{\text{avoid}})$ \COMMENT{Create the root node in the BnB tree.}
    \STATE $\calQ = \calQ.\text{push}(\text{RootNode})$ \COMMENT{Put the root node in the queue.}
    \STATE $l_{\text{unsolved}} = 0$ \COMMENT{Smallest depth where at least one node is unsolved in Figure \ref{fig:BnB_diagram}}
    \WHILE[Keep searching until the time limit is reached or there is no node in the queue.]{$\calQ \neq \emptyset $ and $T_{\text{elapsed}} < T_{\max}$} 
        \STATE $\text{Node} = \calQ\text{.getNode}()$
        \STATE $\calL_{\text{lower}} = \text{Node.lowerSolveFast()}$ \COMMENT{Get the lower bound for this node through the fast method}
        \IF{$\calL_{\text{lower}} < \calL_{\text{best}}^{\text{upper}}$}
            \STATE $\calL_{\text{lower}} = \text{Node.lowerSolveTight()}$ \COMMENT{Get a tighter lower bound for this node through the subgradient ascent}
        \ENDIF
        \IF{$\calL_{\text{lower}} \geq \calL_{\text{best}}^{\text{upper}}$}
            \STATE \textbf{continue} \COMMENT{Prune Node if its lower bound is higher than or equal to the best upper bound.}
        \ENDIF
        \IF{All nodes in depth $l_{\text{unsolved}}$ of the BnB tree are solved}
            \STATE $\calL_{\text{lower}}^{\text{best}} = \max_q(\{\calL^q, \text{for } q \in \{1, 2, ..., l_{\text{unsolved}}\})$ \COMMENT{Tighten the best lower bound; $\calL^q$ is the smallest lower bound of all nodes in depth $q$}
            \STATE $l_{\text{unsolved}} = l_{\text{unsolved}} + 1$ \COMMENT{Raise up the smallest unsolved depth by 1}
            \STATE $\epsilon_{\text{best}} = (\calL_{\text{upper}}^{\text{best}} - \calL_{\text{lower}}^{\text{best}})/\vert{\calL_{\text{upper}}^{\text{best}}}$
            \IF{$\epsilon_{\text{best}} < \epsilon$}
                \STATE \textbf{return} $\bbeta_{\text{best}}$ \COMMENT{Optimality gap tolerance is reached, return the current best solution}
            \ENDIF
        \ENDIF
        \STATE $\bbeta_{\text{upper}}, \calL_{\text{upper}} = \text{Node.upperSolve()}$ \COMMENT{Get feasible sparse solution and its loss from beam search, which is an upper bound for our BnB tree.}
        \IF{$\calL_{\text{upper}} < \calL_{\text{upper}}^{\text{best}}$}
            \STATE $\calL_{\text{upper}}^{\text{best}}, \bbeta_{\text{upper}}^{\text{best}} = \calL_{\text{upper}}, \bbeta_{\text{upper}}$ \COMMENT{Update our best solution and best upper bound}
            \STATE $\epsilon_{\text{best}} = (\calL_{\text{upper}}^{\text{best}} - \calL_{\text{lower}}^{\text{best}})/\vert{\calL_{\text{upper}}^{\text{best}}}$
            \IF{$\epsilon_{\text{best}} < \epsilon$}
                \STATE \textbf{return} $\bbeta_{\text{best}}$ \COMMENT{Optimality gap tolerance is reached, return the current best solution}
            \ENDIF
        \ENDIF
        \STATE $j = \text{Node.getBranchCoord}(\bbeta_{\text{upper}})$ \COMMENT{Get which feature coordinate to branch}
        \STATE $\text{ChildNode1} = \text{CreateNode}(\calD, k, \lambda_2, (\text{Node} \rightarrow \calN_{\text{select}}) \cup \{j\}, \text{Node} \rightarrow \calN_{\text{avoid}})$ \COMMENT{New child node where feature $j$ must be selected}
        \STATE $\text{ChildNode2} = \text{CreateNode}(\calD, k, \lambda_2, \text{Node} \rightarrow \calN_{\text{select}}, (\text{Node} \rightarrow \calN_{\text{avoid}}) \cup \{j\} )$ \COMMENT{New child node where feature $j$ must be avoided}
        \STATE $\calQ \text{.push}(\text{ChildNode1}, \text{ChildNode2})$ \COMMENT{Put the two newly generated nodes into our queue.}
    \ENDWHILE
    \STATE \textbf{return} $\bbeta_{\text{best}}$ \COMMENT{Return the current best solution when time limit is reached or there is no node in the queue}
\end{algorithmic}
\end{algorithm}
